Computing Power of Hybrid Models in Synchronous Networks

During the last two decades, a small set of distributed computing models for networks have emerged, among which LOCAL, CONGEST, and Broadcast Congested Clique (BCC) play a prominent role. We consider hybrid models resulting from combining these three models. That is, we analyze the computing power of models allowing to, say, perform a constant number of rounds of CONGEST, then a constant number of rounds of LOCAL, then a constant number of rounds of BCC, possibly repeating this figure a constant number of times. We specifically focus on 2-round models, and we establish the complete picture of the relative powers of these models. That is, for every pair of such models, we determine whether one is (strictly) stronger than the other, or whether the two models are incomparable. The separation results are obtained by approaching communication complexity through an original angle, which may be of independent interest. The two players are not bounded to compute the value of a binary function, but the combined outputs of the two players are constrained by this value. In particular, we introduce the XOR-Index problem, in which Alice is given a binary vector $x\in\{0,1\}^n$ together with an index $i\in[n]$, Bob is given a binary vector $y\in\{0,1\}^n$ together with an index $j\in[n]$, and, after a single round of 2-way communication, Alice must output a boolean $\textrm{out}_A$, and Bob must output a boolean $\textrm{out}_B$, such that $\mbox{out}_A\land\mbox{out}_B = x_j\oplus y_i$. We show that the communication complexity of XOR-Index is $\Omega(n)$ bits.

==> BBvsS.tex <==
% !TEX root = main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $\ell \geq 1$. We define a language that belongs to $\B^{\ell}$ but does not belong to $\L^*\B^{\ell-1}$. Let us consider the language {\tt $\ell$-pointer-chasing-on-long-path ($\ell$-PCLP)} as the set of paths of length $n$, where the two endpoints of the path have yes instance $\ell$ pointer chasing problem. 
Formally,

\begin{align*}
\mbox{\tt $\ell$-PCLP} = \Big \{(G, \ell) :&\;  \big (\ell:V(G)  \rightarrow \{0,1\}^* \cup \{\perp\}\big) ~\land~\big( G \mbox{ is a path with endpoints } u, v \big) \\
& \land \big( \ell(w) = \perp ~\wedge~ {\tt  \ell-pointer-chasing}(\ell(u),\ell(v)) = 1 \big)\Big \}.
\end{align*}

We have that $\ell$-{\tt PCLP} belongs to $B^\ell$. Indeed, a simple algorithm consists in all vertices communicating its degree in the first round, and at the same time the two endpoints of the path communicating the successive evaluations of $f$. Once $f^\ell(0)$ is computed, every node accepts if (1) all except two nodes have degree $2$, and the two remaining nodes have degree $1$ (hence the graph is a path), and (2) the number of $1$ bits in the binary representation of $f^\ell(0)$ is $1$. 

We now show that $\ell$-{\tt PCLP} does not belong to $\L^*\B^{\ell-1}$. By contradiction, let us suppose that for some $k\geq 0$ there exists an $\epsilon$-error $\L^k\B^{\ell-1}$ algorithm $\mathcal{A}$ for $\ell$-{\tt PCLP}. Given an instance $(f_A, f_B)$ of $\ell$-{\tt pointer chasing}, we define an instance $(P_n, \ell^*)$ of $\ell$-{\tt PCLP} as follows. First, consider on an $2n$-node ($n>k$)  path together endpoints $u$ and $v$. Second, assign $\ell(w) = \perp$ to every node except the endpoints. Third, assign $\ell(u) = f_A$ and $\ell(v)=f_B$. We call $P^u_t$ and $P^v_t$ the set of nodes at distance at most $t$ from $u$ and $v$, respectively.  Observe that $(P_n, \ell^*)$ belongs to $\ell$-{\tt PCLP} if and only if $(f_A, f_B)$ belongs to $\ell$-{\tt pointer-chasing}.

Now consider the following $\epsilon$-error two-player $\ell-1$-round algorithm $\Pi$ for $\ell$-{\tt pointer chasing}. Alice and Bob virtually construct the input $(P_n, \ell^*)$. We say that Alice owns the nodes in $P^u_k$ and Bob owns the nodes $P^v_k$. All nodes that are not owned by Alice or Bob are called \emph{remaining nodes}. The nodes simulate the $k$ {\local} rounds of $\mathcal{A}$ on the nodes they own and on the remaining nodes.  Notice that the players can simulate these rounds without any communication, since the information of the endpoints are at distance $2n > 2k$. Then, the players perform $\ell-1$ rounds of communication. On the $i$-th round, Alice and Bob simulate the $i$-th {\bcc} round of $\mathcal{A}$ on all the nodes they own, generating a packages of messages $M^i_A$ and $M^i_B$, respectively. Then, they communicate $M^i_A$ and $M^i_B$ to each other. Finally, each player simulate the $i$-th  {\bcc} round of $\mathcal{A}$ on the remaining nodes generating a package of messages $M^i_R$ . Observe that these latter messages can be generated as they depend only on the messages sent on the previous rounds, and not on the inputs of $f_A$ and $f_B$. Finally, Alice and Bob have each the packages of messages $M^1, \dots, M^{\ell-1}$ corresponding to the $\ell-1$ {\bcc} rounds of $\mathcal{A}$. Using that information the players can simulate the output of all nodes they own, as well as the output of the remaining nodes. The players then accept in $\Pi$ if and only if all the nodes they own and the remaining nodes accept in $\mathcal{A}$. By the correctness of $\mathcal{A}$, we obtain that with probability $1-\epsilon$, all the nodes in $\mathcal{A}$ accept if and only if Alice and Bob accept in $\Pi$. We deduce that $\Pi$ is an $\ell-1$-round, $\epsilon$-error protocol for $\ell$-{\tt pointer-chasing}. However,  in protocol  Alice and Bob communicate $\cO(\ell k \log n) = \cO(\log n)$ bits, which contradicts Proposition \ref{xx}. We deduce that $\ell$-{\tt PCLP} does not belong to $\L^*\B^{\ell-1}$.


==> preliminaries.tex <==
% !TEX root = main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\emph{Information complexity.}
We now introduce some basic definitions and tools on information complexity. Let $(\Omega, \mu)$ be a discrete probability space. Given a random variable $X$ we denote by $p_X: \Omega \mapsto \mathbb{R}$ the discrete density function of $X$, i.e., $p_X(x) = \text{Pr}(X =x).$ We denote by $H: \omega \mapsto \mathbb{R}^{+}$ the entropy function given by $H(X) = \sum \limits_{x\in \Omega} p_X(x) \frac{1}{\log p_X(x)}.$ We given two random variables $X,Y$ in $\Omega$, we denote by $H(X|Y) = \mathbb{E}_{p_Y(y)}(H(X|Y=y))$ to the entropy of $X$ conditioned to $Y.$ 

Let $\mu$ and $\nu$ be two probability measures in $\Omega.$ The \emph{total variation distance} between $\ mu$ and $\nu$ is given by $|u-v|_{\text{TV}} = \sup \limits_{E\subseteq \Omega} |\mu(E) - \nu(E)|.$ It is well known that  $|u-v|_{\text{TV}} = \frac{1}{2}\sum\limits_{\omega \in \Omega} |\mu(\omega)-\nu(\omega)|$ \textbf{TODO: ref.} In addition, we define the \emph{KL-divergence} (or simply the divergence) between $\mu$ and $\nu$ as $D(\mu||\nu) = \sum \limits_{\omega \in \Omega} \mu(\omega) \log \frac{\mu(\omega)}{\nu(\omega)}.$ Finally, we have that given two random variables $X$ and $Y$ we can define its mutual information as $I(X;Y) = D(p_{X,Y}||p_{X}p_{Y}).$ It is easy to show that $I(X;Y) = H(X) - H(X|Y) = H(Y) - H(Y|X) =I(Y;X).$ Besides, we define the mutual information of $X,Y$ condition to a random variable $Z$ as the function $I(X;Y|Z) = \mathbb{E}_{p_{Z}(z)}[ D(p(\cdot|Z=z)_{X,Y}
||p_{X}(\cdot|Z=z)p_{Y}(\cdot|Z=z))].$ Finally, we present the following technical lemmas that we use during the paper:

\begin{lemma}[Theorem 6.12 \cite{TODO}]
Let $A_1, \hdots, A_n$ be independent random variables and $B$ be jointly distributed then,
$$\sum \limits_{i=1}^{n} I(A_i:B) \leq I(A_1 \hdots, A_n)$$
\end{lemma}
\begin{lemma}[Pinsker's Inequality, Lemma 6.13 \cite{TODO}]
Let $\mu, \nu$ be two probability measures over $\Omega$. Then,   $$|u-v|_{\text{TV}}^2 \leq \frac{2}{\ln 2} D(\mu||\nu)$$
\end{lemma}


